Transferable Embedding Inversion Attack: Uncovering Privacy Risks in Text Embeddings without Model Queries

This study investigates the privacy risks associated with text embeddings, focusing on the scenario where attackers cannot access the original embedding model. Contrary to previous research requiring direct model access, we explore a more realistic threat model by developing a transfer attack method. This approach uses a surrogate model to mimic the victim model's behavior, allowing the attacker to infer sensitive information from text embeddings without direct access. Our experiments across various embedding models and a clinical dataset demonstrate that our transfer attack significantly outperforms traditional methods, revealing the potential privacy vulnerabilities in embedding technologies and emphasizing the need for enhanced security measures.

==> Tables/all_surrogate.tex <==
\begin{table*}[t!]
\centering
\caption{Comparison of embedding inversion performance between different surrogate model. The evaluation are done with embedding models including: OpenAI \texttt{text-embeddings-ada-002}, SBERT~\cite{sentenceBERT} and ST5~\cite{sentence-T5}.}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\multirow{2}{*}{Surrogate / Emb} & \multicolumn{4}{c}{OpenAI} & \multicolumn{4}{c}{SBERT} & \multicolumn{4}{c}{ST5} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
& RougeL & PPL & Cos & LLM-Eval & RougeL & PPL & Cos & LLM-Eval & RougeL & PPL & Cos & LLM-Eval \\
\midrule
\hspace{1em}GTR-base & 0.2071 & 18.692 & 0.4253 & 0.3965 & \textbf{0.1800} & 20.515 & 0.4445 & 0.3899 & 0.1931 & 19.829 & 0.3946 & 0.3743 \\
\hspace{1em}GTR-large & 0.2094 & 18.940 & 0.4234 & 0.3991 & 0.1759 & 19.134 & 0.4505 & 0.3917 & 0.1905 & 19.962 & 0.4028 & 0.3772 \\
\hspace{1em}GTR-xl & 0.2095 & 19.082 & 0.4220 & 0.4047 & 0.1610 & 19.494 & 0.4386 & 0.3843 & 0.1885 & 20.117 & 0.3984 & 0.3759 \\
\hspace{1em}GTR-xxl & 0.2055 & 18.883 & 0.4182 & 0.3983 & 0.1742 & 20.402 & 0.4310 & 0.3686 & 0.1877 & \textbf{18.799} & 0.4019 & 0.3837 \\ \hline
\hspace{1em}ST5-base & 0.1973 & \textbf{17.732} & \textbf{0.4320} & \textbf{0.4071} & 0.1753 & 19.080 & 0.4492 & \textbf{0.3988} & \textbf{0.1948} & 20.656 & 0.3908 & 0.3697 \\
\hspace{1em}ST5-large & 0.2084 & 18.920 & 0.4292 & 0.3986 & 0.1782 & \textbf{19.045} & \textbf{0.4590} & 0.3970 & 0.1913 & 19.917 & 0.4041 & 0.3796 \\
\hspace{1em}ST5-xl & 0.2075 & 18.853 & 0.4211 & 0.3912 & 0.1681 & 19.536 & 0.4398 & 0.3826 & 0.1931 & 20.096 & \textbf{0.4069} & \textbf{0.3840} \\
\hspace{1em}ST5-xxl & \textbf{0.2097} & 18.683 & 0.4303 & 0.3997 & 0.1721 & 19.445 & 0.4379 & 0.3905 & 0.1904 & 20.187 & 0.4024 & 0.3691 \\
\bottomrule
\end{tabular}
}
\label{tab:all_surrogate}
\end{table*}

==> Tables/aug_result.tex <==
% \begin{table}[t!]
% \centering
% \caption{Comparison of embedding inversion performance between different data augmentation approaches. We bold the best performance and underline the second-best performance in the table.}
% \resizebox{\linewidth}{!}{% Resize table to fit the line width
% \begin{tabular}{ccccc}
% \toprule
% Method & RougeL & PPL & Cos & LLM-Eval \\
% \midrule
% LLM & \underline{0.1782} & \textbf{18.062} & \underline{0.4496} & \underline{0.3976} \\
% Swap & \textbf{0.1932} & 35.587 & \textbf{0.5488} & 0.3764 \\
% Delete & 0.1579 & 19.944 & 0.3950 & \textbf{0.4150} \\
% Replace & 0.1727 & 24.991 & 0.4120 & 0.3393 \\
% Insert & 0.1138 & \underline{18.644} & 0.3225 & 0.2387 \\
% \rowcolor{Gray}
% w/o Aug. & 0.1490 & 23.237 & 0.3419 & 0.3270 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:augmentation_result}
% \end{table}

\begin{table}[t!]
\centering
\caption{Comparison of embedding inversion performance between different data augmentation approaches.}
\resizebox{\linewidth}{!}{% Resize table to fit the line width
\begin{tabular}{ccccc}
\toprule
Method & RougeL & PPL & Cos & LLM-Eval \\
\midrule
Transfer + LLM & \textbf{0.1934} & \textbf{10.943} & \textbf{0.4886} & \textbf{0.4276} \\
Direct + LLM & 0.1579 & 20.366 & 0.4525 & 0.3895 \\
Transfer + Replace & 0.1792 & 12.359 & 0.4419 & 0.3563 \\
Direct + Replace & 0.1603 & 19.182 & 0.4124 & 0.3447 \\
\rowcolor{Gray}
Transfer w/o Aug. & 0.1707 & 11.167 & 0.4130 & 0.3511 \\
\rowcolor{Gray}
Direct w/o Aug. & 0.1264 & 27.127 & 0.3257 & 0.3194 \\
\bottomrule
\end{tabular}
}
\label{tab:augmentation_result}
\end{table}

==> Tables/surrogate_result.tex <==
\begin{table}[t!]
\centering
\caption{Comparison of embedding inversion performance between different surrogate model. We bold the best performance in the table.}
\resizebox{\linewidth}{!}{% Resize table to fit the line width
\begin{tabular}{lcccc}
\toprule
Surrogate & RougeL & PPL & Cos & LLM-Eval \\
\midrule
GTR-base & \textbf{0.1800} & 20.515 & 0.4445 & 0.3899 \\
GTR-large & 0.1759 & 19.134 & 0.4505 & 0.3917 \\
GTR-xl & 0.1610 & 19.494 & 0.4386 & 0.3843 \\
GTR-xxl & 0.1742 & 20.402 & 0.4310 & 0.3686 \\ \hline
ST5-base & 0.1753 & 19.080 & 0.4492 & \textbf{0.3988} \\
ST5-large & 0.1782 & \textbf{19.045} & \textbf{0.4590} & 0.3970 \\
ST5-xl & 0.1681 & 19.536 & 0.4398 & 0.3826 \\
ST5-xxl & 0.1721 & 19.445 & 0.4379 & 0.3905 \\
\bottomrule
\end{tabular}
}
\label{tab:surrogate_result}
\end{table}
